Bayesian Networks and Proof-Nets: a proof-theoretical account of Bayesian Inference

We uncover a strong correspondence between Bayesian Networks and (Multiplicative) Linear Logic Proof-Nets, relating the two as a representation of a joint probability distribution and at the level of computation, so yielding a proof-theoretical account of Bayesian Inference.

==> FIGS/macros_figs.tex <==
\usepackage{amsmath, amssymb}
\usepackage{stmaryrd}
\usepackage{proof}

\newcommand{\X}{X^+}
\newcommand{\Xn}{X^-}

\newcommand{\w}{\mathsf{w}}
\newcommand{\cn}{@}
%\newcommand{\cn}{ \mathsf{c}}
%\newcommand{\snode}{\bigtriangledown}

\newcommand{\assoc}{\mathsf {c.ass}}
\newcommand{\neut}{\mathsf {c.w}}
\newcommand{\cid}{\mathsf {c.id}}

\newcommand{\ax}{\mathsf {ax}}
\newcommand{\cut}{\mathsf {cut}}
\newcommand{\bb}{\mathsf {b}}
\newcommand{\true}{\mathtt{t}}
\newcommand{\false}{\mathtt{f}}

\newcommand{\one}{\mathsf {one}}
\newcommand{\bott}{\mathsf {bot}}

\newcommand{\rew}{\rightsquigarrow}

\newcommand{\R}{\mathcal{R}}
%\rightsquigarrow  \looparrowright

%\newcommand{\w}{\bigtriangledown}
%\newcommand{\cn}{\bigtriangledown}

\newcommand{\M}{\mathcal M}
\newcommand{\D}{\mathcal D}

